A Learning Paradigm for Interpretable Gradients

This paper studies interpretability of convolutional networks by means of saliency maps. Most approaches based on Class Activation Maps (CAM) combine information from fully connected layers and gradient through variants of backpropagation. However, it is well understood that gradients are noisy and alternatives like guided backpropagation have been proposed to obtain better visualization at inference. In this work, we present a novel training approach to improve the quality of gradients for interpretability. In particular, we introduce a regularization loss such that the gradient with respect to the input image obtained by standard backpropagation is similar to the gradient obtained by guided backpropagation. We find that the resulting gradient is qualitatively less noisy and improves quantitatively the interpretability properties of different networks, using several interpretability methods.

==> tex/back-1.tex <==
\uppercase{\section{Background}}
\label{sec:back}

%This section presents some background information regarding guided back propagation and CAM methods

% (Need to elaborate, talk about stuff in verbatum like Mythos of Model interpretability)\cite{mythos_interp} GuidedBackprop\cite{guidedbackprop} Deconvnet\cite{deconvnet} Perturbation Model\cite{perturb_inter}

\subsection{Guided backpropagation}
The derivative of the $\relu$ unit $v = \relu(u) = [u]_+ = \max(u,0)$ with respect to its input $u$ is $\ider{v}{u} = \ind_{u>0}$. By the chain rule, a signal $\delta v = \ipder{L}{v}$ is then propagated backwards through $\relu$ to $\delta u = \ipder{L}{u}$ as $\delta u = \ind_{u>0} \delta v$, where the partial derivative of any scalar quantity of interest is meant, \eg a loss $L$.

Guided backpropagation \cite{guidedbackprop} changes this to $\delta_G u = \ind_{u>0} \ind_{dv>0} \delta v = \ind_{u>0} [\delta v]_+$, essentially masking out values corresponding to negative entries of both the forward ($u$) and the backward ($\delta v$) signals and thus preventing backward flow of negative gradients.

Considering the partial derivative $\ipder{L}{u}$ of some loss $L$ with respect to a variable $u$, \eg through an entire network or part of it, standard backpropagation with this particular change for $\relu$ units is called \emph{guided backpropagation}. We denote the corresponding guided ``partial derivative'' or \emph{guided gradient} by $\ipder{_G L}{u}$. This backpropagation method allows sharp visualization of high level activations conditioned on input images.

%------------------------------------------------------------------------------

\subsection{CAM-based methods}

CAM-based methods build a saliency map as a linear combination of  activation map.
Specifically, given a target class $c$ and a set of 2D activation maps $\{A^k\}_{k=1}^K$, % outputed from a convolutional layer of a network,
CAM \cite{cam} is defined as follows:
%ed by $\relu$
\begin{equation}
	S^c = \relu \left( \sum_{k=1}^K \alpha^c_k A^k \right),
\label{eq:cam}
\end{equation}
where the weight $\alpha^c_k$ determines the contribution of channel $k$ to class $c$. This map $S^c$ and the feature maps $A^k$ are non-negative because both are computed with $\relu$ activation functions. Different CAM-based methods differ primarily in the definition of the weights $\alpha^c_k$.

\paragraph{CAM \cite{cam}}
originally defines $\alpha^c_k$ as the weight connecting channel $k$ to class $c$ in the final classifier, assuming $\{A^k\}$ are the feature maps of the last convolutional layer, which is followed by \emph{global average pooling} (GAP) and a single dense layer.

\paragraph{Grad-CAM \cite{gradcam}}

is a generalization of CAM for any networks. If $y^c$ is the logit of class $c$, the weights are obtained by GAP of the partial derivatives of $y^c$ with respect to the feature map $A^k$ of a given layer:
\begin{equation}
    \alpha^c_k = \frac{1}{Z} \sum_{i,j} \pder{y^c}{A^k_{ij}},
\label{eq:gcam}
\end{equation}
where $A^k_{ij}$ denotes the value at spatial location $(i,j)$ of feature map $A^k$ and $Z$ is the total number of locations.

Guided Grad-CAM elementwise-multiplies the saliency maps obtained by Grad-CAM and guided backpropagation, after adjusting spatial resolutions. The resulting visualizations are both class-discriminative (by Grad-CAM) and contain fine-grained detail (by guided backpropagation).

\paragraph{Grad-CAM++ \cite{gradcampp}}

is a generalization of Grad-CAM, where partial derivatives of $y^c$ with respect to $A^k$ are followed by $\relu$ as in guided backpropagation \cite{guidedbackprop} and GAP is replaced by a weighted average:
\begin{equation}
    a^c_k = \sum_{i,j} w^{kc}_{ij} \relu \left( \pder{y^c}{A^k_{ij}} \right).
\label{eq:gcamp}
\end{equation}
The weights $w_{ij}^{kc}$ of the linear combination are
\begin{equation}
    w_{ij}^{kc} = \frac{\pder[2]{y^c}{(A^k_{ij})}}
		{2\pder[2]{y^c}{(A^k_{ij})} + \sum_{a,b} A^k_{ab}\pder[3]{y^c}{(A^k_{ij})}}.
\label{eq:gcampw}
\end{equation}

%\paragraph{Smooth Grad-CAM++ \cite{smoothgradcampp}}

%\green{
%\paragraph{SmoothGrad \cite{smoothgrad}} argues that non-linearities like ReLU activations render derivatives noisy. Thus, to improve smoothness of any derivative $D(x)$ with respect to input image $x$, it takes $m$ Gaussian noise images $\epsilon_i \sim \normal(0,\sigma^2)$ and averages the derivatives with respect to $x + \epsilon_i$:
%\begin{equation}
%    \hat{D}(x) = \frac{1}{m} \sum_{i=1}^m D(x + \epsilon_i).
%\label{eq:smooth}
%\end{equation}
%Smooth Grad-CAM++ \cite{smoothgradcampp} applies this idea to Grad-CAM++ \cite{gradcampp}, essentially replacing all partial derivatives in~\eq{gcamp},\eq{gcampw} by smoothed versions according to~\eq{smooth}.
%}


\paragraph{Score-CAM \cite{scorecam}}

%Following the \emph{increase in confidence} metric proposed in Grad-CAM++,
computes the weights $a^c_k$ based on the increase in confidence \cite{gradcampp} for class $c$ obtained by masking (element-wise multiplying) the input image $x$ with feature map $A^k$:
\begin{equation}
	a^c_k = f(x \circ s(\up(A^k)))_c - f(x_b)_c,
\label{eq:scam}
\end{equation}
where $\up$ is upsampling to the spatial resolution of $x$, $s$ is linear normalization to range $[0,1]$, $\circ$ is the Hadamard product, $f$ is the classifier mapping of input image to class logits and $x_b$ is a baseline image.

While Score-CAM does not require gradients to compute saliency maps, \eq{scam} requires one forward pass through the network $f$ for each channel $k$ and our method modify filters weights during learning.


==> tex/conclusion-1.tex <==
\uppercase{\section{conclusion}}

%\green{TO DO}
In this paper, we propose a new training approach to improve the gradient of a CNN in terms of interpretability.
Our methods forces the gradient obtained from back-propagation at the input image level to align with the gradient coming from guided backpropagation. 
The results of our training are presented according to several metrics and interpretability methods. Our method offers consistent improvement on four out of five metrics for two networks.



==> tex/exp-1.tex <==
\uppercase{\section{Experiments}}

\begin{figure*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{cccccccccc}
    {}&\mr{2}{\Th{Input}}&\mc{2}{\Th{Grad-CAM}}&\mc{2}{\Th{Grad-CAM++}}&\mc{2}{\Th{Score-CAM}}&\mc{2}{\Th{Ablation-CAM}}\\
    {}&{}&\Th{Baseline}&\Th{Denoised}&\Th{Baseline}&\Th{Denoised}&\Th{Baseline}&\Th{Denoised}&\Th{Baseline}&\Th{Denoised}\\
  %  {\rotatebox{90}{\small Man}}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/original/4862.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcam/4862.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcam/4862.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcampp/4862.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcampp/4862.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/scorecam/4862.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/scorecam/4862.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/ablationcam/4862.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/ablationcam/4862.JPEG}\\
    
    {\rotatebox{90}{\small Girl}}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/original/2641.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcam/2641.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcam/2641.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcampp/2641.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcampp/2641.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/scorecam/2641.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/scorecam/2641.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/ablationcam/2641.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/ablationcam/2641.JPEG}\\
    
    {\rotatebox{90}{\small Woman}}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/original/5257.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcam/5257.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcam/5257.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcampp/5257.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcampp/5257.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/scorecam/5257.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/scorecam/5257.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/ablationcam/5257.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/ablationcam/5257.JPEG}\\
        
    {\rotatebox{90}{\small Lobster}}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/original/5160.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcam/5160.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcam/5160.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcampp/5160.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcampp/5160.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/scorecam/5160.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/scorecam/5160.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/ablationcam/5160.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/ablationcam/5160.JPEG}\\
    
    {\rotatebox{90}{\small Couch}}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/original/2043.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcam/2043.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcam/2043.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/gradcampp/2043.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/gradcampp/2043.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/scorecam/2043.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/scorecam/2043.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/baseline/ablationcam/2043.JPEG}&\includegraphics[width=0.09\textwidth]{fig/fig_cam/cosine/ablationcam/2043.JPEG}\\
    
    
\end{tabular}
%\vspace{3pt}
\caption{Saliency map comparison of several CAM-based methods with standard vs our training on CIFAR-100 examples.}
\label{fig:salient}
\end{figure*}

%This section presents the experimental settings, the definition of our evaluation metrics and results.
%Finally, we present qualitative and quantitative results and an ablation study.\\



\subsection{Experimental Set-up}

In the following sections, we evaluate recognition and interpretability capabilities of our approach. 
Specifically, we generate explanations following popular attribution methods derived from CAM \cite{cam}, from the \textbf{pytorch-grad-cam} library from Jacob Gildenblat\footnote{https://github.com/jacobgil/pytorch-grad-cam}.


\paragraph{Models and Dataset}
We train and evaluate a ResNet-18 \cite{he16} and a MobileNet-V2 \cite{sandler2018mobilenetv2} on CIFAR-100 \cite{krizhevsky2009learning}. 
ResNets are the most common CNNs and the 18's is particularly adapted to low resolution images.
MobileNet-V2 is a widely used compact CNN.
CIFAR-100 contains 60.000 images of 100 categories, split in 50.000 for training and 10.000 for testing. Each image has a resolution of $32\times32$ pixels. This dataset is chosen because of its ease of usage and prototyping properties. 

\paragraph{Settings}
To obtain competitive performance and ensure the replicability of our method, we follow the methodology by weiaicunzai \footnote{https://github.com/weiaicunzai/pytorch-cifar100}. Thus, we perform 200 epochs, with a starting learning rate of $10^{-1}$, a batch-size of 128 images, SGD optimizer and a learning rate division by 5 on epochs 60, 120 and 160.  

\subsection{Faithfulness Evaluation}
Faithfulness evaluation via image recognition as proposed in \cite{gradcampp} offers insight about the regions of an image that are considered important for recognition, as highlighted by the saliency map $S^c$. 
Specifically, given a class $c$, an image \textit{I} and a computed saliency map $S^c$ are element-wise multiplied to obtain a masked image $M^c$:

\begin{equation*}
    M^c = S^c\circ I
\end{equation*}

This masked image is similar to the original image on the salient areas and becomes black on the non-salient ones.
To evaluate the saliency maps capability, we forward both the image and the masked version through the network to obtain the prediction scores \textit{$Y_i^c$} and \textit{$O_i^c$} respectively. We then compute the following metrics:

\begin{itemize}
    \item \textbf{Average Drop (AD)} 
    Aims at quantifying how much predictive power is lost when we take into consideration the masked image compared to the original one. Lower is better.
    \begin{equation}
        AD(\%) = \sum_{i=1}^N \frac{max(0,Y_i^c- O_i^c)}{Y_i^c}
    \end{equation}
    \label{Average Drop}
    
    \item \textbf{Average Increase (AI)}
    Unlike Average Drop, Average Increase, also known as Increase of Confidence, measures the percentage of instances of the dataset where the masked image offers a higher score than the original images for a specific class. Higher is better.
    
    \begin{equation}
        AI(\%) = \frac{1}{N} \sum_i^N \mathbbm{1}{(Y_i^c<O_i^c)}*100
    \end{equation}

    \item \textbf{Average Gain (AG)} 
    Recently introduced in Opti-CAM \cite{zhang2023opti}, 
    this metric is designed to be a complement for Average Drop. This measurement is meant to quantify the gain in predictive power attained when the masked image is taken in comparison compared to the original one.
     Higher is better.
    \begin{equation}
        AG(\%) = \sum_{i=1}^N \frac{max(0, O_i^c-Y_i^c)}{Y_i^c}
    \end{equation}
\end{itemize}


\subsection{Causal Metrics for Explanations}
Causality evaluation as proposed in RISE \cite{petsiuk2018rise}, aims at evaluating the effect of masking certain elements of the image and retrieving the change in predictive power for a model. Thus, the authors proposed \textbf{Insertion} and \textbf{Deletion}.

\textbf{Insertion} starts from a blurry image and gradually insert the pixel of the original image ranked in terms of saliency, coming from a given saliency map. At each iteration the images are passed
through the network to compute the prediction ratio compared to the original prediction.

\textbf{Deletion} gradually removes the pixels starting from the most salient ones. Removed pixels are replaced by black and, as for insertion, we compute the prediction at each iteration. Histograms
and average of these metrics can be computed per image. As most previous work we only show the mean insertion and deletion percentages averaged over the test set.


\subsection{Qualitative Experiments}
We visualize the effect of our approach on Figure \ref{fig:salient} and \ref{fig:grads}, which  presents saliency maps, respectively gradient, obtained for the baseline model and the one trained with our approach.
%Conversely, to study the effect of our methodology, on Figure \ref{fig:grads} we demonstrate the differences between the gradients of models trained with our approach and without it.

Regarding saliency maps, we observe the differences brought by our training method that improves interpretability metrics.
The differences are particularly important fro Grad-CAM which directly averages the gradient to weigh feature maps.
Interestingly the differences are smaller on Score-CAM that is not gradient based and only obtains changes from the differences in feature maps.

%that there is some degree of overlapping regarding the higlighted regions for each method, however those differences can be explained in part because of the training procedure performed, given accuracies are different between approaches;

%however, it is important to notice that while accuracy might not always be better, these differences between image parts highlighted lead to gains on interpretable recognition. 
Gradient visualizations show a bit less noise and magnitude with our method.
%On another part, while it has been acknowledged that standard gradients are hard to explain and the information conveyed by them is overall hard to interpret, we observe that our approach indeed leads to less noisy gradients; 
Moreover, the object of interest is better covered by gradient activations. 
%images is presented in a clearer way, thus proving the intended behavior of our training.

\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{cccc}
        {}&\mr{2}{\Th{Input}}&\mc{2}{\Th{Gradient}}\\
        {}&{}&\Th{Baseline}&\Th{Ours}\\
        {\rotatebox{90}{\small Bed}}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/original/5415.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/baseline/5415.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/cosine/5415.JPEG}\\
        
   %     {\rotatebox{90}{\small Lamp}}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/original/1766.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/baseline/1766.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/cosine/1766.JPEG}\\

        {\rotatebox{90}{\small Lawnmower}}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/original/8311.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/baseline/8311.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/cosine/8311.JPEG}\\

        {\rotatebox{90}{\small Maple Tree}}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/original/1198.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/baseline/1198.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/cosine/1198.JPEG}\\

        {\rotatebox{90}{\small Sunflower}}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/original/8881.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/baseline/8881.JPEG}&\includegraphics[width=0.125\textwidth]{fig/fig_grad/cosine/8881.JPEG}\\
    \end{tabular}
    \caption{Visualization of standard gradient with models trained with standard and our approach.}
    \label{fig:grads}
\end{figure}


\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{lcccccc}\\\toprule
        \mc{7}{\Th{\textbf{Recognition Metrics}}}\\\midrule
        \Th{Model}&\Th{Error}& &\Th{$\lambda$}&\Th{Acc}& &\\\midrule
        \mr{2}{\Th{ResNet-18}}&-& &-&\Th{73.42}& &\\
         &\Th{Cosine}& &$7.5\times10^{-3}$&\Th{72.86}& &\\\midrule
         
        \mr{2}{\Th{MobileNet-V2}}&-& &-&\Th{59.43}&\\
         &\Th{Cosine}&  &$1\times10^{-3}$&\Th{62.36}&\\\midrule
        
        \mc{7}{\Th{\textbf{Interpretable Recognition Metrics}}}\\\midrule    
        \mc{7}{\Th{ResNet-18}}\\\midrule
        \Th{Method}&\Th{Error}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{Ins$\uparrow$}&\Th{Del$\downarrow$}\\\hline
        \mr{2}{\Th{Grad-CAM}}&-&30.16&15.23&29.99&58.47&17.47\\
         &\Th{Cosine}&28.09&16.19&31.53&58.76&17.57\\\hline
        \mr{2}{\Th{Grad-CAM++}}&-&31.40&14.17&28.47&58.61&17.05\\
          &\Th{Cosine}&29.78&15.07&29.60&58.90&17.22\\\hline
        \mr{2}{\Th{Score-CAM}}&-&26.49&18.62&33.84&58.42&18.31\\
          &\Th{Cosine}&24.82&19.49&35.51&59.11&18.34\\\hline
        \mr{2}{\Th{Ablation-CAM}}&-&31.96&14.02&28.33&58.36&17.14\\
         &\Th{Cosine}&29.90&15.03&29.61&58.70&17.37\\\hline
        \mr{2}{\Th{Axiom-CAM}}&-&30.16&15.23&29.98&58.47&17.47\\
          &\Th{Cosine}&28.09&16.20&31.53&58.76&17.57\\\midrule

        \mc{7}{\Th{MobileNet-V2}}\\\midrule
        \Th{Method}&\Th{Error}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{Ins$\uparrow$}&\Th{Del$\downarrow$}\\\hline
        \mr{2}{\Th{Grad-CAM}}&-&44.64&6.57&25.62&44.64&14.34\\
         &\Th{Cosine}&40.89&7.31&27.08&45.57&15.20\\\hline
        \mr{2}{\Th{Grad-CAM++}}&-&45.98&6.12&24.10&44.72&14.76\\
          &\Th{Cosine}&40.76&6.85&26.46&45.51&14.92\\\hline
        \mr{2}{\Th{Score-CAM}}&-&40.55&7.85&28.57&45.62&14.52\\
          &\Th{Cosine}&36.34&9.09&30.50&46.35&14.72\\\hline
        \mr{2}{\Th{Ablation-CAM}}&-&45.15&6.38&25.32&44.62&15.03\\
          &\Th{Cosine}&41.13&7.03&26.10&45.38&15.12\\\hline
        \mr{2}{\Th{Axiom-CAM}}&-&44.65&6.57&25.62&44.64&15.27\\
          &\Th{Cosine}&40.89&7.31&27.08&45.57&15.20\\\bottomrule

    \end{tabular}
    \caption{Experiments with cosine error function on CIFAR-100 with ResNet-18 and MobileNet-V2. Accuracy and interpretability metrics are reported.}
    \label{tab:C100_quant}
\end{table}
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{lcccccc}\\\toprule
    \mc{7}{Regularization Selection}\\\midrule
    \Th{Regularizer}&\Th{Acc}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{Ins$\uparrow$}&\Th{Del$\downarrow$}\\\midrule
    - &73.42&30.16&15.23&29.99&58.47&17.47\\
    Cosine&72,86&\textbf{28.09}&\textbf{16.19}&\textbf{31.53}&58.76&17.57\\
    Histogram &73.88&30.39&14.78&29.38&58.52&17.35\\
    MAE & 73,41& 30,33 & 15,06 &29,61 & 58,13 & 17,95\\
    MSE & 73,86& 29,64 & 15,19 &30,11 & \textbf{59,05} & 18,02\\\bottomrule
    \end{tabular}
    \caption{\textbf{Regularization selection: } Evaluation of the four proposed regularization with ResNet-18 on CIFAR-100.}%}
    \label{tab:Regs}
\end{table}

\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{lcccccc}\\\toprule
    \mc{7}{Regularization Selection}\\\midrule
    $\lambda$&\Th{Acc}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{Ins$\uparrow$}&\Th{Del$\downarrow$}\\\midrule
    - &73.42&30.16&15.23&29.99&58.47&17.47\\
    $1\times10^{-3}$ &\textbf{73.71}&29.52&15.17&30.03&59.23&\textbf{17.45}\\
    $2.5\times10^{-3}$ &72.99&30.53&15.82&30.56&59.04&17.96\\
    $5\times10^{-3}$ &72.46&30.10&16.06&30.67&57.47&17.80\\
    $7.5\times10^{-3}$ &72.86&\textbf{28.09}&\textbf{16.20}&\textbf{31.53}&58.76&17.57\\
    $1\times10^{-2}$ &73.28&28.97&15.75&31.16&58.99&17.50\\
    $1\times10^{-1}$ &73.00&28.93&16.13&31.55&\textbf{59.66}&17.95\\
    $1$ &73.30&28.44&16.02&31.31&58.64&17.48\\
    $10$ &73.04&29.28&15.23&30.47&58.74&17.47\\\bottomrule
    \end{tabular}
    \caption{\textbf{Regularization coefficient:} Evaluation of the regularization coefficient $\lambda$, using ResNet-18 with \textit{Cosine Similarity} on CIFAR-100.}%}
    \label{tab:variation}
\end{table}

\subsection{Quantitative Experiments}
We evaluate the effect of training a given model using our proposed approach with \textit{Faithfulness} and \textit{Causality}. Results are reported in Table \ref{tab:C100_quant}.

As we see, we obtain improvements on both networks and systematically on five out of six metrics. 
The improvements are higher for AD, AG, and AI. 
Insertion gets a smaller but consistent improvement and Deletion is almost always worst with our method, but with a very small difference.
This decrease in Deletion may be due to some limitations of the metrics, as reported in previous works \cite{zhang2023opti}.

It is interesting to note that improvements on Score-CAM means that our training not only improves gradient but also builds better activation maps, since Score-CAM only rely on those.




\subsection{Ablation Experiments}
We conduct ablation experiments using ResNet18. In these experiments we analyze the different regularization proposals mentioned in Section \ref{sec:method} and the impact of the regularization coefficient.

\paragraph{Regularization proposals} 
To validate our selection of regularization function, we train several models following the same training regime while varying the error function. To evaluate these approaches, we focus solely on Grad-CAM attributions. Results are reported in Table \ref{tab:Regs}




Following these results, we observe a consistent improvement on most metrics for all regularizer options. 
We note that the accuracy remains stable within half a percent of the original model.
However, we note that most options struggle regarding deletion. 
Cosine Similarity however manages to provide improvements in most metrics, while maintaining deletion performance.
 
\paragraph{Regularization coefficient}
Finally we study the behavior of the regularization coefficient $\lambda$ in \ref{eq:total}. We train multiple models with \textit{Cosine Similarity} and a range of values for $\lambda$, see Table \ref{tab:variation}.

We observe that our method is not very sensible to the regularization coefficient and that the value of $7.5e^{-3}$ offers better performances and is thus selected as the default value for $\lambda$.





==> tex/intro-1.tex <==
\uppercase{\section{Introduction}}
%\section{Introduction}



The improvements of deep learning methods in the last decade has led to very large developments and a large diffusion to most sectors. Since these models are computationally complex and opaque, the requirements for explanations or interpretable models receives a lot of attention nowadays \cite{mythos_interp}. Explanations and transparency becomes a legal requirements for diverse types of systems that are used to assist high-stakes decisions.


In this work, we study deep learning models visual interpretability.
Model interpretability is often categorized into transparency or post-hoc methods. Transparency aims at producing interpretable models where the inner process or part of it can be understood. Post-hoc methods consider models as black-boxes and interpret decisions mainly based on inputs and outputs.
Regarding visual recognition models
a few models include some transparency using concepts or parts \cite{sicre23}, but most methods focus on post-hoc interpretability with saliency maps. These maps highlight the most important areas of an image related to the decision.
Initial works focused on gradient information such as guided back-propagation \cite{guidedbackprop}.
CAM \cite{cam} later presented a class-specific linear combination of feature maps that opened the way to numerous weighting strategies.
Several methods use gradient information \cite{gradcam}, masking \cite{scorecam}, etc.
GradCAM \cite{gradcam} and other variants \cite{omeiza2019smooth} are particularly successful gradient methods.
Interestingly SmoothGrad \cite{smoothgrad} and SmoothGrad-CAM++ \cite{omeiza2019smooth} improve the precision of saliency maps by denoising gradient.
%These CAM-based methods are the most popular and best performing methods at the moment.

In this work, we follow a similar idea and propose a learning paradigm for model training that constraint gradient in order to improve the performance of interpretability methods.
In fact, we add a regularization term to the loss function pulling the gradient in the input space to align with the values obtained by guided back-propagation.
Such regularization has a smoothing effect on gradient and is expected to improve the precision of model interpretations.


More specifically the Figure \ref{fig:method} summarizes our method.
When training each input image is forwarded to the network to compute the cross-entropy loss. Then a standard and guided back-propagations are computed back to the input image space, where our regularization term is computed. This term is added to the loss and back-propagated only through the standard back-propagation branch.



The key contributions of this learning interpretable gradients approach follows:
\begin{itemize}
    \item We introduce a new learning framework with regularized gradient.
    \item The proposed method is further evaluated on several architectures both in term of accuracy and interpretability metrics.
\end{itemize}



%------------------------------------------------------------------------------
\begin{figure*}[t]
\centering
% \fig[0.45]{method}

%------------------------------------------------------------------------------
\begin{tikzpicture}[
	scale=.3,
	font={\footnotesize},
	node distance=.5,
	label distance=3pt,
	wide/.style={yscale=.75},
	net/.style={draw,trapezium,trapezium angle=75,inner sep=3pt},
	enc/.style={net,shape border rotate=270},
	dec/.style={net,shape border rotate=90},
	txt/.style={inner sep=3pt},
	loose/.style={looseness=.6},
	sg/.style={blue!60},
]
\matrix[
	tight,row sep=6,column sep=16,
	cells={scale=.3,},
] {
	\&\&\&\&\&
	\node[dec] (guided-back) {guided \\ backprop}; \&
	\node[wide,label=90:$\ipder{_G L_C}{x}$] (guided) {\fig[.1]{method/guided_gradient}}; \\
	\node[label=90:input image $x$] (in) {\fig[.1]{method/input}}; \&
	\node[enc] (net) {network \\ $f$}; \&\&\&
	\node[box] (class) {classification \\ loss $L_C$}; \&
	\node[dec] (back) {standard \\ backprop}; \&
	\node[wide,label=90:$\ipder{L_C}{x}$] (grad) {\fig[.1]{method/gradient}}; \&
	\node[box] (reg) {regularization \\ loss $L_R$}; \\
	\&\&\&\&\&\&\&
	\node[op] (plus) {$+$}; \&
	\node[txt] (loss) {total loss \\ $L = L_C + $\\ $\lambda L_R$}; \\
};

\draw[->]
	(in) edge (net)
	(net) edge node[above] {logits $y$} (class)
	(class) edge (back)
	(back) edge (grad)
	(guided-back) edge[sg] (guided)
	(grad) edge (reg)
	(reg) edge (plus)
	(plus) edge (loss)
	(class) edge[sg,out=90,in=180] (guided-back)
	(class) edge[loose,out=-50,in=180] (plus)
	(guided) edge[sg,out=0,in=90] node[pos=.2,font=\large,label=0:stop gradient] {//} (reg)
	(net) edge[dashed,out=60,in=150] (guided-back)
	(net) edge[dashed,out=30,in=150] (back)
	;

\end{tikzpicture}
%------------------------------------------------------------------------------

\caption{Proposed interpretable gradient learning. For an input image $x$, we obtain the logit vector $y = f(x; \theta)$ by a forward pass through the network $f$ with parameters $\theta$. We compute the classification loss $L_C$ by softmax and cross-entropy~\eq{class}, \eq{ce}. We obtain standard gradient $\ipder{L_C}{x}$ and guided gradient $\ipder{_G L_C}{x}$ by two backward passes
%, after stopping the gradient of the latter,
and compute the regularization loss $L_R$ as the error between the two~\eq{reg},\eq{mae}-\eq{cos}.
%We thus learn to denoise the standard gradient according to the guided one.
Finally, the total loss is $L = L_C + \lambda L_R$~\eq{total}.
%Backpropagation through $f$ is depicted ``unrolled'' as a decoder; there are implicit connections between the forward and backward passes (dashed lines).
Learning is based on $\ipder{L}{\theta}$, which involves differentiation of the entire computational graph except the guided backpropagation branch (in blue).}
\label{fig:method}
\end{figure*}
%------------------------------------------------------------------------------



==> tex/method-1.tex <==
\uppercase{\section{Proposed method}}
\label{sec:method}

\paragraph{Preliminaries}

We consider an image classification network $f$ with parameters $\theta$, which maps an input image $x$ to a vector of class logits $y = f(x; \theta)$. At inference, we predict the class label of maximum confidence $\arg\max_j y_j$, where $y_j$ is the logit of class $i$. At training, given training images $X = \{x_i\}_{i=1}^n$ and target labels $T = \{t_i\}_{i=1}^n$, we compute the \emph{classification loss}
\begin{equation}
	L_C(X, \theta, T) = \frac{1}{n} \sum_{i=1}^n \ce(f(x_i; \theta), t_i),
\label{eq:class}
\end{equation}
where $\ce$ is softmax followed by cross-entropy:
\begin{equation}
	\ce(y, t) = -\log \frac{e^{y_t}}{\sum_i e^{y_i}} = -y_t + \sum_i e^{y_i}.
\label{eq:ce}
\end{equation}
Updates of parameters $\theta$ are then performed by an optimizer, based on the standard partial derivative (gradient) $\ipder{L_C}{\theta}$ of the classification loss $L_C$ with respect to $\theta$,  obtained by standard back-propagation.

However, due to non-linearities like ReLU activations and downsampling like max-pooling or convolution stride $> 1$, the standard gradient is noisy \cite{smoothgrad}. This is show by visualizing the gradient $\ipder{L_C}{x}$ with respect to an input image $x$. By contrast, the guided gradient $\ipder{_G L_C}{x}$ \cite{guidedbackprop} does not suffer much from noise and preserves sharp details. The difference of the two gradients is illustrated in \ref{fig:method}.

\paragraph{Regularization}

The main idea of this work is to introduce a regularization term during training, which will make the standard gradient $\ipder{L_C}{x}$ behave similarly to the corresponding guided gradient $\ipder{_G L_C}{x}$, while maintaining the predictive power of the classifier $f$. We hypothesize that, if possible, this will improve the quality of all gradients with respect to intermediate activations and therefore the quality of saliency maps obtained by CAM-based methods \cite{cam,gradcam,gradcampp,scorecam} and the interpretability of network $f$. The effect may be similar to that of SmoothGrad \cite{smoothgrad}, but without the need for several forward passes at inference.

In particular, given an input image $x$, we perform a forward pass through $f$ and compute the logit vectors $y_i = f(x_i, \theta)$ and the classification loss $L_C(X, \theta, T)$~\eq{class}. We then obtain the standard gradients $\delta x_i = \ipder{L_C}{x_i}$ and the guided gradients $\delta_G x_i = \ipder{_G L_C}{x_i}$ with respect to the input images $x_i$ by two separate backward passes. Since the whole process is differentiable (\wrt $\theta$) at training, we stop the gradient computation of the latter, so that it only serves as a ``teacher''. We define the \emph{regularization loss}
\begin{equation}
	L_R(X, \theta, T) = \frac{1}{n} \sum_{i=1}^n E(\delta x_i, \delta_G x_i),
\label{eq:reg}
\end{equation}
where $E$ is an error function between the two gradient images, considered below.

Finally, the total loss is defined as
\begin{equation}
	L(x, \theta, t) = L_C(x, \theta, t) + \lambda L_R(x, \theta, t),
\label{eq:total}
\end{equation}
where $\lambda$ is a hyperparameter determining the regularization coefficient.
$\lambda$ should be large enough to smooth the gradient without decreasing the classification accuracy or hurting the training process.
Updates of the network parameters $\theta$ are now based on the gradient $\ipder{L}{\theta}$ \wrt the total loss, using any optimizer. At inference, one may use any interpretability method to obtain a saliency map at any layer.

\paragraph{Algorithm}
Our method is summarized in Algorithm \ref{alg:grad} %, where \textsc{detach} stops gradient computation,
and illustrated in \ref{fig:method}.It is interesting to note that the entire computational graph depicted in \ref{fig:method} involves one forward and two backward passes. This graph is then differentiated again to compute $\ipder{L}{\theta}$, which involves one more forward and backward pass, since the guided backpropagation branch is excluded. Thus, each training iteration requires five passes through $f$ instead of two in a standard training.
%------------------------------------------------------------------------------
\begin{algorithm}
	\SetFuncSty{textsc}
	\SetDataSty{emph}
	\newcommand{\commentsty}[1]{{\color{DarkGreen}#1}}
	\SetCommentSty{commentsty}
	\SetKwComment{Comment}{$\triangleright$ }{}

	\SetKwFunction{Detatch}{detatch}

	\KwIn{network $f$, parameters $\theta$}
	\KwIn{input images $X = \{x_i\}_{i=1}^n$}
	\KwIn{target labels $T = \{t_i\}_{i=1}^n$}
	\KwOut{loss $L$}
	$L_C \gets \frac{1}{n} \sum_i \ce(f(x_i; \theta), t_i)$ \Comment*[f]{class. loss \eq{class}} \\
    \ForEach{$i \in \{1,\dots,n\}$}{
	 	$\delta_G x_i \gets \ipder{_G L_C}{x_i}$ \Comment*[f]{guided grad} \\
        $\mbox{\Th{Detach}}(\delta_G x_i)$ \Comment*[f]{detach from graph}
	 	$\delta x_i \gets \ipder{L_C}{x_i}$ \Comment*[f]{standard grad} \\
	  }
   $L_R \gets \frac{1}{n} \sum_{i=1}^n E(\delta x_i, \delta_G x_i) $ \Comment*[f]{reg. loss \eq{reg}}
 $L \gets L_C + \lambda L_R$
 \Comment*[f]{total loss ~\eq{total}} \\

\caption{Interpretable gradient loss}
\label{alg:grad}
\end{algorithm}
%------------------------------------------------------------------------------


 %This amounts to $2.5\times$ computation overhead.

%\green{is it 2.5 times in space too ???}

\paragraph{Error function}

Given two gradient images $\delta, \delta'$ consisting of $p$ pixels each, we consider the following error functions $E$ to compute the regularization loss~\eq{reg}.


%\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=3pt]
%    \item Sigmoid Masking
%    \begin{equation}
%        E_{\sigma}(\delta,\delta') = - \sum_{i=0}^p \delta'\odot\frac{e^{\delta}}{e^{\delta}+1}.
%    \end{equation}
%    \item Centered Sigmoid Masking
%    \begin{equation}
%        E_{\sigma}(\delta,\delta') = - \sum_{i=0}^p \delta'\odot\frac{e^{\delta-\mu_\delta}}{e^{\delta-\mu_\delta}+1}.
%    \end{equation}
%\end{enumerate}


\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=3pt]

 	\item Mean absolute error:
 	\begin{equation}
 		E_{\mae}(\delta, \delta') = \frac{1}{p} \norm{\delta - \delta'}_1.
 	\label{eq:mae}
\end{equation}
 	\item Mean squared error:
 	\begin{equation}
 		E_{\mse}(\delta, \delta') = \frac{1}{p} \norm{\delta - \delta'}_2^2.
 	\label{eq:mse}
 	\end{equation}

\end{enumerate}

We also consider the following two similarity functions, with a negative sign.
\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=3pt]
	\setcounter{enumi}{2}
	\item Cosine similarity:
	\begin{equation}
		E_{\cos}(\delta, \delta') = -\frac{\inner{\delta, \delta'}}{\norm{\delta}_2 \norm{\delta'}_2},
	\label{eq:cos}
	\end{equation}

	\item Histogram intersection:
	\begin{equation}
		E_{\hi}(\delta, \delta') = -\sum_{i=0}^p
			\frac{\min(\abs{\delta_i}, \abs{\delta'_i})}{\norm{\delta}_1 \norm{\delta'}_1}.
	\label{eq:hi}
	\end{equation}

	where $\inner{,}$ denotes inner product.

\end{enumerate}

% \begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=3pt]
% 	\item Mean absolute error:
% 	\begin{equation}
% 		E_{\mae}(\delta, \delta') = \frac{1}{p} \norm{\delta - \delta'}_1.
% 	\label{eq:mae}
% 	\end{equation}
% 	\item Mean squared error:
% 	\begin{equation}
% 		E_{\mse}(\delta, \delta') = \frac{1}{p} \norm{\delta - \delta'}_2^2.
% 	\label{eq:mse}
% 	\end{equation}
% \end{enumerate}

% We also consider the following two similarity functions, with a negative sign.

%\green{Do we mention the changes in the architecture so the }


==> tex/plots-ext.tex <==
%------------------------------------------------------------------------------
% hack for CVPR/ICCV style
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikzextern}
\usepackage{pgffor}

%------------------------------------------------------------------------------
% externalization
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/rel-1.tex <==
\section{\uppercase{Related Work}}

% Begining of interpretability, basics
Interpretability and explainability of DNN decisions is a topic that receives increasing interest.
As interpretability is not a simple notion to define, Lipton \cite{mythos_interp} proposes some common ground, definitions and categorization for interpretability methods.
For instance, transparency aims at making models simple so it is humanly possible to provide an explanation of its inner mechanism.
However, post-hoc method consider models as black boxes and study the activations leading to a specific output.
LIME \cite{LIME} and SHAP \cite{NIPS2017_7062} are probably the most popular post-hoc methods that are model agnostic and provide local information.
Concerning CNN addressing image recognition tasks, numerous work generate saliency maps highlighting the areas of an image that are responsible for a specific decision.
Many of these methods are either based on back-propagation and its variant or on Class Activation Maps (CAM) that weight the importance of activation maps.



% Link to the families/approaches towards interpretability
%As a first approach towards model interpretability, we take notice at what it is and why is it important. %No sentence like that
% Restructuring, stuff like mythos of interpretability, definitions, concept
%%%%%%Restructuring in order with Topics:
%\textbf{Study on Activations maps}
%This approach towards interpreting models, considers interpretations as activations of a given network, on the input space for a model. Some of the earlier works \cite{deconvnet,understanding_visz} laid the basis upon understanding what deeper layers on a model have learn, while building class-specific saliency maps by gradient ascent on the input space.
%% LIME?

\subsection{Gradient-based approaches}
%\cite{guidedbackprop}\cite{smoothgrad}\cite{cam}
Gradient-based approaches assess the impact of distinct image regions on the prediction based on the partial derivative of the model's prediction function with respect to the input. A simple saliency map can be the partial derivatives obtained in one gradient backward pass through the model~\cite{simonyan2013deep}. 
Meanwhile, \emph{Guided backpropagation}~\cite{guidedbackprop} enhances explanations by nullifying negative gradients through the use of ReLU units.
For better visualization, \emph{SmoothGrad}~\cite{smoothgrad} introduce noise-multiplication techniques applied to the input, deriving saliency maps based on the mean of resultant gradients.
%\emph{Integrated gradients (IG)}~\cite{sundararajan2017axiomatic} estimates the importance of image regions by approximating the integral from the baseline images to the inputs via a Riemann sum.
\emph{Layer-wise Relevance Propagation (LRP)}~\cite{bach2015pixel} reallocates the prediction score through a custom backward pass across the network.% with a local conservation principle. 
%LRP is further substantiated via Deep Taylor Decomposition~\cite{montavon2017explaining,montavon2018methods} to provide additional justification for its methodology.



%\textbf{Latent Space based approaches}


\subsection{CAM-based approaches} Class Activation Maps \cite{cam} is a method that produces a saliency map that highlights the areas of an image that are the most responsible for a CNN decision. 
The map is computed as a linear combinations of feature maps from a given layer and predicted category.
Different variants of CAM are proposed by modifying the weighting coefficients for a given activation map. Grad-CAM \cite{gradcam}, for instance, computes the averaged gradient back-propagated from a given class. 
It is also possible to extend this principle to multiple layers \cite{layercam} and 
to improve sensitivity \cite{sundararajan2017axiomatic} and conservation \cite{montavon2018methods} by the addition of axioms towards the computation \cite{axiombased}. Moreover, Grad-CAM++ \cite{gradcampp}  improves the object localization capabilities by leveraging positive partial derivatives and measuring interpretability with recognition and localization metrics. 
As mentioned earlier, the gradient can be further improved by adding noise \cite{smoothgrad}. %\cite{omeiza2019smooth}. 
Later, Score-CAM \cite{scorecam} proposes a gradient-free method that compute weighting coefficients maximizing the Average Increase metric \cite{gradcampp}. 
%Further improvements are proposed by adding integration to compute scores \cite{iscam}, applying the denoising idea \cite{sscam}.
%, or 
Further improvements are proposed using instance level optimization \cite{zhang2023opti}. 
Finally, some works provide explanations that not only are good at localizing salient parts on images, but also provide theoretical bases on the effect of modifying such regions for a given input \cite{axiombased}.
An exhaustive alternative  performs ablation experiments to highlight such parts \cite{ramaswamy2020ablation}.



%\cite{layercam,axiombased},\cite{gradcampp,smoothgcpp} \cite{scorecam,iscam}







%In his work, Lipton\cite{mythos_interp} suggests that the term interpretability is ill-defined, however it has a purpose being that of conveying useful information about the processes of decision making for any given model; thus its relevance comes from the need about knowing what leads these processes, and the demand of explanation when there is a mismatch between the formal objectives of supervised learning and the costs of deployment in the real world. Complementary to these ideas, Selvaraju \etal \cite{gradcam} implies that interpretability is important, as it is required to build trust upon intelligent systems as they are moving towards meaningful integration to our daily lives; thus, we find essential to be able to explain what they predict.\\
%
%Complementary to his proposals, Lipton proposes that an interpretable model should be \textit{transparent} \ie \textit{for a given model a complete explanation of how it works is expected} and be able to provide \textit{post-hoc} explanations \ie \textit{insight of the activations that lead a model towards a given output}. It is also noted by Lipton that the concept of interpretability is both important but plastic; and in that regard several considerations are given towards the claims of qualification interpretability, the possibility of mislead from post-hoc interpretations amongst others.\\
%How do we observe interpretability
%From the previously enunciated properties of interpretability, special attention has been taken into post-hoc explanations; in due part because \textit{interpretations} provided by it do not compromise predictive performance, but also because this concept aligns with what humans deem interpretable. In computer vision, this sort of interpretability is most often applied by generating visualizations on the input space to qualitatively observe what a model has learned. For this goal, two attributes of a CNN model can be studied: the activations for a given signal, and the gradient that said signal produces on them; moreover it is also possible to induct perturbations on to the inputs to observe changes in predictive power, while on another hand it is also possible to work with features on the latent space, understanding how a change in them affects the predictive power or it can be seen on the input space\cite{networkdecoupling,disentangling_latent}.\\% Regarding activations, we observe some of the earlier works\cite{deconvnet,LIME},\\
%One of the first proposals to better understand the predictions of CNN, Zieler\& Fergus proposed the deconvolution\cite{deconvnet}; highlighting parts of an image that strongly activate a neuron. Complementary to this, Springenberg \etal \cite{guidedbackprop} proposed the \textit{guided backpropagation}, which helps understanding the impact of each neuron \wrt an image. \cite{LIME}\\
% Should it be split on gradient-based methods, saliency methods?
% Why do we want to measure it
%To be able to measure interpretability, it is necessary to quantify it; on this regard, Bau \etal\cite{dissection} propose to consider the task as that of detection, thus they compute the intersection over union \textit{IoU} for all of the activations of a convolutional unit in a CNN, and the annotation mask for a given concept, on their Boden dataset. Amongside this approach, we also find that human evaluation is often used to estimate this \cite{cam, detectors_emergence}. Most recently, more quantifiable methods towards measuring interpretability have been   %% Add more
%\noindent\textbf{CAM-based approaches}
%Throw papers inside. Check notes from reading list.

% Define what interpretability is, why is important, talk about mythos of model interpretability, BRODEN maybe
% Base interpretability approaches, focus on saliency, deconvnet, 
%Transparency/Posthoc interpretability
%Distillation
%Particular interest in CNN interpretability
% CAM-based approaches-> Saliency
% then cam
%Deconvolution
%Guided Backpropagation \cite{guidedbackprop}
%CAM, identifying discriminative regions
%

% Other interpretability approaches, Thislooks like that, network decoupling
% Interpretability approaches

%\noindent Our proposed approach presents an opportunity to improve upon the previously mentioned methods, where by denoising the gradient flowing through the network, we can obtain cleaner activations at a given layer.\\
%\textbf{What is Interpretability? Benchmarks, Mythos of Model interpretability; first approaches} \cite{mythos_interp}\cite{dissection}first approaches \cite{visualizing&saliency,deconvnet} make interpretability reasoning like humans process information \cite{lookslikethat} 
% \textbf{Interpretability approaches, gradient based, saliency based, decoupling based}  \cite{guidedbackprop} \cite{smoothgrad}; \textbf{Deep Interpretable models} \cite{recognition_grouping} \textbf{Latent Space}latest, investigating through latent space\cite{senseofcnns}

% \textbf{CAM based approaches} \cite{cam} \cite{gradcam} Then comes Grad-CAM\cite{gradcam}, a derivation with layercam and axiom-based cam\cite{layercam,axiombased} then gradcam++\cite{gradcampp}, derivations with \cite{smoothgradcampp} then we talk about score-cam \cite{scorecam}\cite{smoothgcpp}

% \textbf{How do we measure interpretability?}
%Our approach is complementary to both Grad-CAM and Grad-CAM++, as these proposals rely on the gradient flowing through the network to obtain activations, thus learning to obtain cleaner gradients can porduce better activations. In contrast with Smooth-Grad and Smooth Grad-CAM++, our approach aims to learn how to denoise these gradients, \textbf{JUSTIFY WHY IS THIS BETTER THAN JUST ADDING NOISE TO DENOISE}; finally, compared to Score-CAM, our approach distills knowledge from the gradient cleaning process, into producing better activation maps, additionally, the insight gathered during the training phase of our approach can be used to complement Score-CAM. \textbf{DIFFERENCES TO SCORE-CAM}





\subsection{Double backpropagation}
Double backpropagation is a general regularization method first introduced by Drucker and Le Cun \cite{drucker1991double} to improve generalization.
The idea is later used to avoid overfitting \cite{philipp2018nonlinearity}, help transfer \cite{srinivas2018knowledge}, cope with noisy labels \cite{luo2019simple}, and recently to increase adversarial robustness \cite{lyu2015unified,simon2018adversarial,ross2018improving,seck20191,finlay2018improved}.
This regularization aims at penalizing the \emph{L1} \cite{seck20191}, \emph{L2}, or \emph{L$\infty$} norm of the gradient with respect to the input image.
%and can also be refered as Jacobian penalty. 

Our method is related and regularizes the gradient by aligning standard and guided gradient.


%Double back prooften used for adversarial training.
%In most cases one uses some norm of the gradient \wrt the input image as a loss. 
%Our contribution is that we use some norm of the difference between standard and guided gradient instead.


%Adv:
%l2 norm in Finlay
%
%luo: something different: regularizaiton is variance of prediction according to some perturbation to cope with noisy labels Jacobian
%
%Lyu:
%l2 and l infinity like finlay
%fast gradient sign method
%
%Philipp: nonlinearity coefficient to predict overfitting.
%
%Ros gradient wrt to input
%
%Seck l1 norm
%
%Drucket improve generalization l2
%
%Simon first double for adversarial ?
%
%Srinivas
%Jacobian-based penalties improve distillation, robustness to noisy inputs, and transfer learnin

